High-order expansion of Neural Ordinary Differential Equations flows

Artificial neural networks, widely recognised for their role in machine learning, are now transforming the study of ordinary differential equations (ODEs), bridging data-driven modelling with classical dynamical systems and enabling the development of infinitely deep neural models. However, the practical applicability of these models remains constrained by the opacity of their learned dynamics, which operate as black-box systems with limited explainability, thereby hindering trust in their deployment. Existing approaches for the analysis of these dynamical systems are predominantly restricted to first-order gradient information due to computational constraints, thereby limiting the depth of achievable insight. Here, we introduce Event Transition Tensors, a framework based on high-order differentials that provides a rigorous mathematical description of neural ODE dynamics on event manifolds. We demonstrate its versatility across diverse applications: characterising uncertainties in a data-driven prey-predator control model, analysing neural optimal feedback dynamics, and mapping landing trajectories in a three-body neural Hamiltonian system. In all cases, our method enhances the interpretability and rigour of neural ODEs by expressing their behaviour through explicit mathematical structures. Our findings contribute to a deeper theoretical foundation for event-triggered neural differential equations and provide a mathematical construct for explaining complex system dynamics.

==> figures/siren.tex <==
\def\layersep{2cm}
\def\nodesep{0.7cm}
\def\linewidthact{0.18mm}
\definecolor{americanrose}{rgb}{1.0,0.01,0.24}
\definecolor{or}{rgb}{1.0,0.49,0.0}
\definecolor{yell}{rgb}{1.0,0.75,0.0}

% Define a command to select one of three colors randomly
\newcommand{\randomcolor}{
    \pgfmathsetmacro{\randnum}{int(random(1,3))}
    \ifnum\randnum=1
        \def\colorselect{americanrose}
    \else\ifnum\randnum=2
        \def\colorselect{or}
    \else
        \def\colorselect{yell}
    \fi\fi
}
% Define the hidden neuron softplus style to include the random color selection
\newcommand{\hiddenneuronrandomcolor}{
    \randomcolor
    \tikzstyle{hidden neuron softplus}=[neuron_hidden, fill=\colorselect]
}

\begin{tikzpicture}[shorten >=1pt,->,draw=black!50, node distance=\layersep, scale=1]
    % \tikzstyle{every pin edge}=[<-,shorten <=1pt]
    \tikzstyle{every pin edge}=[<-,shorten <=1pt,line width=0.5pt,color=black!85, opacity=0.5]


    \tikzset{mystyle/.style={line width=0.025mm,color=black!75, opacity=0.5}}

    \tikzstyle{neuron}=[circle,fill=black!25,minimum size=6pt,inner sep=0pt]

    \tikzstyle{neuron_hidden}=[circle,fill=black!25,minimum size=8pt,inner sep=0pt]
    
    \tikzstyle{input neuron}=[neuron, fill=gray];
    \tikzstyle{output neuron}=[neuron, fill=blue];
    \tikzstyle{output neuron2}=[neuron, fill=blue];

    \tikzstyle{hidden neuron softplus}=[neuron_hidden, fill=blue!50];

    \tikzstyle{annot} = [text width=4em, text centered]

    % Draw the input layer nodes
    \node[input neuron, pin=left:$$] (I-1) at (0,-\nodesep*1*1.2) {};
    \node[input neuron, pin=left:$$] (I-2) at (0,-\nodesep*2*1.2) {};
    \node[input neuron, pin=left:$$] (I-3) at (0,-\nodesep*3*1.2) {};
    \node[input neuron, pin=left:$$] (I-4) at (0,-\nodesep*4*1.2) {};
    \node[input neuron, pin=left:$$] (I-5) at (0,-\nodesep*5*1.2) {};
    % \node[] (L0) at (0,-\nodesep*7*1.63-4.6*\nodesep) {$L^{(0)}$};


    % Draw the hidden layer 1 nodes
    \foreach \name / \y in {1,...,16}
        \hiddenneuronrandomcolor
        \path[yshift=0.5cm]
            node[hidden neuron softplus] (H1-\name) at (\layersep,-\nodesep*0.5*\y) {};
    % \node[] (L1) at (\layersep,-\nodesep*15-1*\nodesep) {$L^{(1)}$};

            
    % Draw the hidden layer 2 nodes
    \foreach \name / \y in {1,...,16}
        \hiddenneuronrandomcolor
        \path[yshift=0.5cm]
            node[hidden neuron softplus] (H2-\name) at (1.8*\layersep,-\nodesep*0.5*\y) {};
    % \node[] (L2) at (2*\layersep,-\nodesep*15-1*\nodesep) {$L^{(2)}$};
            
    % Draw the hidden layer 3 nodes
    \foreach \name / \y in {1,...,16}
        \hiddenneuronrandomcolor
        \path[yshift=0.5cm]
            node[hidden neuron softplus] (H3-\name) at (2.6*\layersep,-\nodesep*0.5*\y) {};
    % \node[] (Ll) at (2.5*\layersep,-\nodesep*15-1*\nodesep) {$L^{(l)}$};

    % Draw the output neurons
    \node[output neuron2, pin={[pin edge={->}]right:$$}, right of=H3-3] (O-1) at (2.3*\layersep,-1.6)  {};
    \node[output neuron2, pin={[pin edge={->}]right:$$}, right of=H3-3] (O-2) at (2.3*\layersep,-2)  {};
    \node[output neuron2, pin={[pin edge={->}]right:$$}, right of=H3-3] (O-3) at (2.3*\layersep,-2.4)  {};
    \node[output neuron2, pin={[pin edge={->}]right:$$}, right of=H3-3] (O-4) at (2.3*\layersep,-2.8)  {};
    % \node[below of=O-2] (Ll1) at (3.8*\layersep,-6.6*\nodesep) {$L^{(l+1)}$};

    \pgfdeclarelayer{background}
    \pgfsetlayers{background,main}
    % Connect every node in the input layer with every node in the
    % hidden layer2.

    % Begin background layer
    \begin{pgfonlayer}{background}

    \foreach \source in {1,...,5}
        \foreach \dest in {1,...,16}
            \path[mystyle] (I-\source) edge (H1-\dest);
            
    % Connect every node in the hidden layer1 with the hidden layer 2
    \foreach \source in {1,...,16}
        \foreach \dest in {1,...,16}
            \path[mystyle] (H1-\source) edge (H2-\dest);

    % % Draw the dots for the missing layers      
    % \path[thick] ([xshift=.1cm] H2-8.east) edge[-,loosely dotted] ([xshift=.1cm] H3-8.east);

    % Connect every node in the hidden layer1 with the hidden layer 3
    \foreach \source in {1,...,16}
        \foreach \dest in {1,...,16}
            \path[mystyle] (H2-\source) edge (H3-\dest);

    % Connect every node in the hidden layer 3 with the output layer
    \foreach \source in {1,...,16}
        \foreach \dest in {1,...,4}
            \path[mystyle] (H3-\source) edge (O-\dest);



    \end{pgfonlayer}
    

    \pgfmathsetmacro{\scale}{0.2}
    \pgfmathsetmacro{\Ox}{10}
    \pgfmathsetmacro{\Oy}{4}

    % Plot nonlinearities
    \draw[scale=\scale, shift = {(\Ox, \Oy)}] (-3,0) -- (4,0) node[right] {};
    \draw[scale=\scale, shift = {(\Ox, \Oy)}] (0,-1) -- (0,3) node[above] {};
    \draw[-, scale=\scale,domain=-3:3,smooth,variable=\x,yell, shift = {(\Ox, \Oy)} ] 
        plot ({\x},{sin(1 * \x r)});
    % Second sine wave with double the frequency
    \draw[-, scale=\scale,domain=-3:3,smooth,variable=\x,or, shift = {(\Ox, \Oy)} ] 
        plot ({\x},{sin(2 * \x r)});
    % Third sine wave with triple the frequency
    \draw[-, scale=\scale,domain=-3:3,smooth,variable=\x,americanrose, shift = {(\Ox, \Oy)}, line width=\linewidthact ] 
        plot ({\x},{sin(3 * \x r)});
    
    \draw[scale=\scale, shift = {(\Ox+8, \Oy)}] (-3,0) -- (4,0) node[right] {};
    \draw[scale=\scale, shift = {(\Ox+8, \Oy)}] (0,-1) -- (0,3) node[above] {};
    \draw[-, scale=\scale,domain=-3:3,smooth,variable=\x,yell, shift = {(\Ox+8, \Oy)}, line width=\linewidthact ] 
        plot ({\x},{sin(1 * \x r)});
    % Second sine wave with double the frequency
    \draw[-, scale=\scale,domain=-3:3,smooth,variable=\x,or, shift = {(\Ox+8, \Oy)}, line width=\linewidthact ] 
        plot ({\x},{sin(2 * \x r)});
    % Third sine wave with triple the frequency
    \draw[-, scale=\scale,domain=-3:3,smooth,variable=\x,americanrose, shift = {(\Ox+8, \Oy)}, line width=\linewidthact ] 
        plot ({\x},{sin(3 * \x r)});
    
    \draw[scale=\scale, shift = {(\Ox+16, \Oy)}] (-3,0) -- (4,0) node[right] {};
    \draw[scale=\scale, shift = {(\Ox+16, \Oy)}] (0,-1) -- (0,3) node[above] {};
    \draw[-, scale=\scale,domain=-3:3,smooth,variable=\x,yell, shift = {(\Ox+16, \Oy)}, line width=\linewidthact ] 
        plot ({\x},{sin(1 * \x r)});
    % Second sine wave with double the frequency
    \draw[-, scale=\scale,domain=-3:3,smooth,variable=\x,or, shift = {(\Ox+16, \Oy)}, line width=\linewidthact ] 
        plot ({\x},{sin(2 * \x r)});
    % Third sine wave with triple the frequency
    \draw[-, scale=\scale,domain=-3:3,smooth,variable=\x,americanrose, shift = {(\Ox+16, \Oy)}, line width=\linewidthact ] 
        plot ({\x},{sin(3 * \x r)});
    
   
    % The sigmoid
    \draw[scale=\scale, shift = {(\Ox+27.25, \Oy-6.5)}] (0,-1) -- (0,3) node[above] {};
    \draw[-,scale=\scale,domain=-2:2,smooth,variable=\x,blue, shift = {(\Ox+27, \Oy-6.5)}, line width=\linewidthact ] plot ({\x},{1/(1+exp(-\x * 2))});
    
    % \draw[scale=\scale, shift = {(\Ox+30, \Oy-15)}] (-1,0) -- (3,0) node[right] {};
    % \draw[scale=\scale, shift = {(\Ox+30, \Oy-15)}] (0,-1) -- (0,3) node[above] {linear};
    % \draw[scale=\scale,domain=-2:3,smooth,variable=\x,green, shift = {(\Ox+30, \Oy-15)} ] plot ({\x},{(\x)});
    
    % \node[above, align=center, font=\bfseries] at (current bounding box.north) {Asteroid landing};
        %\draw[scale=\scale,domain=-3:3,smooth,variable=\x,red, shift = {(\Ox, \Oy)} ] plot ({\x},{tanh(\x)});
\end{tikzpicture}

% \caption{Drone racing - Full G\&CNET architecture.} \label{fig:ffnn_drone}

% \end{figure}

==> figures/siren2.tex <==
\def\layersep{2cm}
\def\nodesep{0.7cm}
\def\linewidthact{0.18mm}
\definecolor{americanrose}{rgb}{1.0,0.01,0.24}
\definecolor{or}{rgb}{1.0,0.49,0.0}
\definecolor{yell}{rgb}{1.0,0.75,0.0}

% Define a command to select one of three colors randomly
\newcommand{\randomcolor}{
    \pgfmathsetmacro{\randnum}{int(random(1,3))}
    \ifnum\randnum=1
        \def\colorselect{americanrose}
    \else\ifnum\randnum=2
        \def\colorselect{or}
    \else
        \def\colorselect{yell}
    \fi\fi
}
% Define the hidden neuron softplus style to include the random color selection
\newcommand{\hiddenneuronrandomcolor}{
    \randomcolor
    \tikzstyle{hidden neuron softplus}=[neuron_hidden, fill=\colorselect]
}

\begin{tikzpicture}[shorten >=1pt,->,draw=black!50, node distance=\layersep, scale=1]
    % \tikzstyle{every pin edge}=[<-,shorten <=1pt]
    \tikzstyle{every pin edge}=[<-,shorten <=1pt,line width=0.5pt,color=black!85, opacity=0.5]


    \tikzset{mystyle/.style={line width=0.025mm,color=black!75, opacity=0.5}}

    \tikzstyle{neuron}=[circle,fill=black!25,minimum size=6pt,inner sep=0pt]

    \tikzstyle{neuron_hidden}=[circle,fill=black!25,minimum size=8pt,inner sep=0pt]
    
    \tikzstyle{input neuron}=[neuron, fill=gray];
    \tikzstyle{output neuron}=[neuron, fill=blue];
    \tikzstyle{output neuron2}=[neuron, fill=blue];

    \tikzstyle{hidden neuron softplus}=[neuron_hidden, fill=blue!50];

    \tikzstyle{annot} = [text width=4em, text centered]

    % Draw the input layer nodes
    \node[input neuron, pin=left:$$] (I-1) at (0,-\nodesep*2*1.2) {};
    \node[input neuron, pin=left:$$] (I-2) at (0,-\nodesep*3*1.2) {};
    \node[input neuron, pin=left:$$] (I-3) at (0,-\nodesep*4*1.2) {};
    % \node[] (L0) at (0,-\nodesep*7*1.63-4.6*\nodesep) {$L^{(0)}$};


    % Draw the hidden layer 1 nodes
    \foreach \name / \y in {1,...,16}
        \hiddenneuronrandomcolor
        \path[yshift=0.5cm]
            node[hidden neuron softplus] (H1-\name) at (\layersep,-\nodesep*0.5*\y) {};
    % \node[] (L1) at (\layersep,-\nodesep*15-1*\nodesep) {$L^{(1)}$};

            
    % Draw the hidden layer 2 nodes
    \foreach \name / \y in {1,...,16}
        \hiddenneuronrandomcolor
        \path[yshift=0.5cm]
            node[hidden neuron softplus] (H2-\name) at (1.8*\layersep,-\nodesep*0.5*\y) {};
    % \node[] (L2) at (2*\layersep,-\nodesep*15-1*\nodesep) {$L^{(2)}$};
            
    % Draw the hidden layer 3 nodes
    \foreach \name / \y in {1,...,16}
        \hiddenneuronrandomcolor
        \path[yshift=0.5cm]
            node[hidden neuron softplus] (H3-\name) at (2.6*\layersep,-\nodesep*0.5*\y) {};
    % \node[] (Ll) at (2.5*\layersep,-\nodesep*15-1*\nodesep) {$L^{(l)}$};

    % Draw the output neurons
    \node[output neuron2, pin={[pin edge={->}]right:$$}, right of=H3-3] (O-1) at (2.3*\layersep,-2.4)  {};
    % \node[below of=O-2] (Ll1) at (3.8*\layersep,-6.6*\nodesep) {$L^{(l+1)}$};

    \pgfdeclarelayer{background}
    \pgfsetlayers{background,main}
    % Connect every node in the input layer with every node in the
    % hidden layer2.

    % Begin background layer
    \begin{pgfonlayer}{background}

    \foreach \source in {1,...,3}
        \foreach \dest in {1,...,16}
            \path[mystyle] (I-\source) edge (H1-\dest);
            
    % Connect every node in the hidden layer1 with the hidden layer 2
    \foreach \source in {1,...,16}
        \foreach \dest in {1,...,16}
            \path[mystyle] (H1-\source) edge (H2-\dest);

    % % Draw the dots for the missing layers      
    % \path[thick] ([xshift=.1cm] H2-8.east) edge[-,loosely dotted] ([xshift=.1cm] H3-8.east);

    % Connect every node in the hidden layer1 with the hidden layer 3
    \foreach \source in {1,...,16}
        \foreach \dest in {1,...,16}
            \path[mystyle] (H2-\source) edge (H3-\dest);

    % Connect every node in the hidden layer 3 with the output layer
    \foreach \source in {1,...,16}
        \foreach \dest in {1}
            \path[mystyle] (H3-\source) edge (O-\dest);



    \end{pgfonlayer}
    

    \pgfmathsetmacro{\scale}{0.2}
    \pgfmathsetmacro{\Ox}{10}
    \pgfmathsetmacro{\Oy}{4}

    
   
    % \draw[scale=\scale, shift = {(\Ox+30, \Oy-15)}] (-1,0) -- (3,0) node[right] {};
    % \draw[scale=\scale, shift = {(\Ox+30, \Oy-15)}] (0,-1) -- (0,3) node[above] {linear};
    % \draw[scale=\scale,domain=-2:3,smooth,variable=\x,green, shift = {(\Ox+30, \Oy-15)} ] plot ({\x},{(\x)});
    
    % \node[above, align=center, font=\bfseries] at (current bounding box.north) {Asteroid landing};
        %\draw[scale=\scale,domain=-3:3,smooth,variable=\x,red, shift = {(\Ox, \Oy)} ] plot ({\x},{tanh(\x)});
\end{tikzpicture}

% \caption{Drone racing - Full G\&CNET architecture.} \label{fig:ffnn_drone}

% \end{figure}
